Psychophysical Evaluation of Deep Re-Identification Models

Pedestrian re-identification (ReID) is the task of continuously recognising the sameindividual across time and camera views. Researchers of pedestrian ReID and theirGPUs spend enormous energy producing novel algorithms, challenging datasets,and readily accessible tools to successfully improve results on standard metrics.Yet practitioners in biometrics, surveillance, and autonomous driving have not re-alized benefits that reflect these metrics. Different detections, slight occlusions,changes in perspective, and other banal perturbations render the best neural net-works virtually useless. This work makes two contributions. First, we introducethe ReID community to a budding area of computer vision research in model eval-uation. By adapting established principles of psychophysical evaluation from psy-chology, we can quantify the performance degradation and begin research thatwill improve the utility of pedestrian ReID models; not just their performance ontest sets. Second, we introduce NuscenesReID, a challenging new ReID datasetdesigned to reflect the real world autonomous vehicle conditions in which ReIDalgorithms are used. We show that, despite performing well on existing ReIDdatasets, most models are not robust to synthetic augmentations or to the morerealistic NuscenesReID data.

==> chapters/Glossary.tex <==
\chapter*{Glossary of Terms}
\label{glossary}
\begin{longtable}{r p{0.6\textwidth}}
    \textbf{\textit{Complicated Term}}: & Make sure to define anything that you allude to in the text\\
    \textbf{\textit{Parameter}}: & Description of the parameter. This is not the same as the List of Symbols. \\
\end{longtable}

==> chapters/Journals.tex <==
\chapter*{List of Journal Abbreviations}
% I have included a list of common journals that are used in Biostatistics. Make sure that your .bib file abbreviations match what is here. - HG 2018
\begin{center}
\begin{longtable}{lp{0.56\textwidth}}
  Am J Epidemiol \dotfill & American Journal of Epidemiology \\
  Am J Public Health \dotfill & American Journal of Public Health \\
  Am Stat \dotfill & The American Statistician \\
  Ann Intern Med \dotfill & Annals of Internal Medicine \\
  Ann Stat \dotfill & The Annals of Statistics \\
  Arch Intern Med \dotfill & Archives of Internal Medicine \\
  BMJ \dotfill & The British Medical Journal \\
  Can J Stat \dotfill & The Canadian Journal of Statistics \\
  IEEE Trans Automat Contr \dotfill & Institute of Electrical and Electronics Engineers Transactions on Automatic Control \\
  JAMA \dotfill & Journal of the American Medical Association \\
  JASA \dotfill & Journal of the American Statistical Association \\
  J R Stat Soc Ser B \dotfill & Journal of the Royal Statistical Society. Series B (Statistical Methodology) \\
  J R Stat Soc Ser C \dotfill & Journal of the Royal Statistical Society. Series C (Applied Statistics) \\
  J Stat Softw \dotfill & The Journal of Statistical Software \\
  N Engl J Med \dotfill & New England Journal of Medicine \\
  Stat Med \dotfill & Statistics in Medicine 
\end{longtable}
\end{center}


==> chapters/Symbols.tex <==
\chapter*{List of Symbols and Abbreviations}\label{RefSymbols}
  \begin{longtable}{lp{0.75\textwidth}}
    AIC \dotfill & Akaike's Information Criterion \\
    CI \dotfill & Confidence Interval \\
    CP \dotfill & Coverage Probability \\
    HR \dotfill & Hazard Ratio \\
	PLR \dotfill & Pooled Logistic Regression\\
\end{longtable}
